QuadTree Attention for Vision Transformers

Transformers have been successful in many vision tasks, thanks to their capability of capturing long-range dependency. However, their quadratic computational complexity poses a major obstacle for applying them to vision tasks requiring dense predictions, such as object detection, feature matching, stereo, etc. We introduce QuadTree Attention, which reduces the computational complexity from quadratic to linear. Our quadtree transformer builds token pyramids and computes attention in a coarse-to-fine manner. At each level, the top K patches with the highest attention scores are selected, such that at the next level, attention is only evaluated within the relevant regions corresponding to these top K patches. We demonstrate that quadtree attention achieves state-of-the-art performance in various vision tasks, e.g. with 4.0% improvement in feature matching on ScanNet, about 50% flops reduction in stereo matching, 0.4-1.5% improvement in top-1 accuracy on ImageNet classification, 1.2-1.8% improvement on COCO object detection, and 0.7-2.4% improvement on semantic segmentation over previous state-of-the-art transformers. The codes are available at https://github.com/Tangshitao/QuadtreeAttention.

==> iclr2022/complexity.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{l|llllll}
           & Linear & Reduction-(8,8) & Quadtree-1 & Quadtree-4 & Quadtree-8 & Quadtree-16 \\ \hline
Complexity & $O(NC^2)$ & $O(KNC)$           & $O(KNC)$     & $O(KNC)$      & $O(KNC)$      & $O(KNC)$       \\ \hline
Flops      & 0.63   & 0.16            & 0.04       & 0.11      & 0.16       & 0.28       
\end{tabular}
\caption{Computation complexity and flops of linear attention, reduction attention and quadtree attention. We assume the token size is $60\times 80$} and the key tokens and value tokens of reduction attention is $8\times 8$
\end{table}

==> iclr2022/detection_table_old.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{l|lllllll}
                & Flops (G) & AP   & $AP_{50}$ & $AP_{75}$ & $AP_S$ &$AP_M$ &$AP_L$  \\ \hline
ResNet18 (\cite{he2016deep})   & 38.6  & 31.8 & 49.6 & 33.6 & 16.3 & 34.3 & 43.2 \\
PVTv2-b0 (\cite{wang2021pvtv2})        & 28.3  & 37.2 & 57.2 & 23.1& 40.4 & 49.6 & 49.7 \\
% Quadtree-A-b0 (K=8, ours) & \textbf{14.7}  & 36.8 & 56.8 & 38.7& 22.3 &39.7 &49.1 \\
% \sout{Quadtree-B-b0 (K=8, ours) \jiahui{delete}} & 15.0  & 37.1 & 56.9 & 39.4& 22.5& 39.8& \textbf{50.1} \\
QuadTree-A-b0 (K=32, ours)  & \textbf{16.0}  & 37.0 & 56.8 & 38.9& \textbf{22.8}&
39.7& 50.0 \\
QuadTree-B-b0 (K=32, ours) & 16.5  & \textbf{37.5} & \textbf{57.7} & \textbf{39.6}& 22.4&\textbf{40.5} &49.9 \\ \hline
ResNet50 (\cite{he2016deep})       &  87.3 & 36.3 & 55.3 & 38.6& 19.3 & 40.0 & 48.8 \\
PVTv1-Tiny (\cite{wang2021pyramid})       & 72.5  & 36.7 & 56.9 & 38.9& 22.6 & 38.8 & 50.7 \\
PVTv2-B1 (\cite{wang2021pvtv2})       & 78.8  & 41.2 & 61.9 & 43.9& 25.4 & 44.5 & 54.3 \\
%\sout{Quadtree-B-b1 (K=8, ours)\jiahui{delete}}  & \textbf{52.5}  &41.1 &61.8      &43.7& 24.7 &44.9 &54.3     \\
Quadtree-B-b1 (K=32, ours) & \textbf{56.2}  &\textbf{41.4}  &\textbf{62.2}  &\textbf{44.0}& \textbf{25.8}&
\textbf{45.4}& \textbf{54.4}    \\ \hline
ResNet101 (\cite{he2016deep})       &  166.3 & 38.5 &  57.8 & 41.2&  21.4 &  42.6 &  51.1 \\
ResNeXt101-32x4d (\cite{xie2017aggregated})       & 170.2 & 39.9 & 59.6 &  42.7& 22.3 &  44.2 & 52.5 \\
PVTv1-small (\cite{wang2021pyramid})       & 139.8  & 36.7 & 56.9 & 38.9& 25.0 & 42.9 &  55.7 \\
PVTv2-B2 (\cite{wang2021pyramid})     & 149.1 &44.6 &65.6  &47.6& 27.4 & 48.8 & 58.6 \\
%\sout{Quadtree-B-b2 (K=8, ours)\jiahui{delete}}  & \textbf{102.0}  &44.5 &65.4  &47.7& 27.8& 48.5& 58.3      \\
QuadTree-B-b2 (K=32, ours) & \textbf{108.6}  & \textbf{44.9}& \textbf{66.2} &\textbf{47.7}& \textbf{28.9} &\textbf{49.2} &\textbf{58.9}
\end{tabular}
\caption{Object detection results on COCO val2017 with RetinaNet. We use PVTv2 backbone and replace the reduction attention with quadtree attention. `Flops' is the backbone flops for input image size of $800\times 1,333$.}
\vspace{-5mm}
\label{tab:detection}
\end{table}

==> iclr2022/flow.tex <==
\subsubsection{Optical flow Estimation}
Optical flow aims to estimate per-pixel motion between video frames. RAFT (\citep{teed2020raft}) is the state-of-the-art optical flow estimation method. It first extracts image features, builds 4D cost volumes for all pairs of pixels, and iteratively updates a flow field through GRU (\citep{cho2014properties}). There is no transformer-based method for this task. Therefore, we simply add 4 (self+cross) transformer blocks after the feature extractor and still use RAFT framework to estimate the optical flow, but unfortunately there is no notable improvement in common used datasets like Sintel and Kitti. We think their performance  to has been saturated because the motions of Sintel and Kitti is small and using transformer do not bring any performance gain. As a result, we construct a new dataset from ScanNet (\cite{dai2017scannet}) that contains large displacement flow. 

\textbf{Setting.} We mainly compare quadtree attention with linear attention (\citep{katharopoulos2020transformers}) and spatial reduction attention (\citep{wang2021pyramid}). For spatail reduction attention, we also average pooling the key and value to the size of $8\times 8$. The architecture of the block is the same as the one used in LoFTR. For training, we use the data to train LoFTR-lite. We resize the image to 480*640 and train the model with a batch size of 8 on 4 2080TI GPU for 200000 iterations. We set the base learning rate to 0.0004. For testing, we random sample xx pairs with frame interval smaller than 80 from the ScanNet testing video. We use the standard metric end-point-error (EDE) to evaluate our method.

\input{iclr2022/flow_table}

\textbf{Results.} Table. \ref{tab:flow} shows the end-point-error for RAFT, RAFT with linear attention, RAFT with spatial reduction attention and RAFT with quadtree attention. We list the performance under different average ground truth flow magnitude. The first row "Avg GT" means the average flow value of one pair is smaller than some value, e.g. 50. We also list the number of pairs below. In the table, it is unusual that linear attention obtain worse performance than the baseline. We do not further explore the reason and leave it for future work.
For spatial reduction attention and quadtree attention-A, they obtain similar performance as baseline. In contrast, quadtree attention-B outperform all those methods, which reduces the end point error from 5.43 to 5.27. It is also noted that quadtree attention-B has more advantages in estimating large displacement flow than the RAFT baseline. For example, the EDE is nearly the same when the average magnitude is less than 50, but the EDE reduced from 6.94 to 6.55 when the average flow magnitude is 100-150. 

==> iclr2022/flow_table.tex <==
% \begin{table}[]
% \centering
% \begin{tabular}{@{}l|lllll@{}}
% Avg GT      & 0    & 100  & 200   & 300   & All   \\
% Pair number & 1525 & 1406 & 930   & 534   & 4395  \\ \midrule
% RAFT        & 4.20 & 8.41 & 12.40 & 34.49 & 10.96 \\ \midrule
% Linear      & 4.12 & 8.61 & 12.82 & 36.31 & 11.31 \\ \midrule
% Reduction   & 4.09 & 8.58 & 12.35 & 34.29 & 10.94 \\ \midrule
% Quadtree-A8 & 4.19 & 8.33 & 11.95 & 31.82 & 10.51 \\ \midrule
% Quadtree-B8 & 4.14 & 8.21 & 12.26 & 28.94 & 10.19
% \end{tabular}
% \caption{\ping{put some description in the caption. This experiment is quite questionable. I never see optical flow been evaluated on images with such a large GT flow magnitude.}}
% \end{table}

% \begin{table}[]
% \begin{tabular}{@{}l|lllllllll@{}}
% Avg GT      & 0    & 50   & 100  & 150  & 200   & 250   & 300   & 350   & All   \\
% Pair number & 731  & 794  & 773  & 633  & 538   & 392   & 309   & 225   & 4744  \\ \cmidrule(r){1-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(l){10-10} 
% RAFT        & 2.83 & 5.46 & 7.87 & 9.06 & 11.63 & 13.43 & 22.57 & 50.98 & 10.96 \\ \cmidrule(r){1-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(l){10-10} 
% Linear      & 2.84 & 5.31 & 7.82 & 9.89 & 11.52 & 13.45 & 24.52 & 56.16 & 11.31 \\ \cmidrule(r){1-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(l){10-10} 
% Reduction   & 2.79 & 5.29 & 7.77 & 9.59 & 11.60 & 13.43 & 21.65 & 51.69 & 10.94 \\ \cmidrule(r){1-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(l){10-10} 
% Quadtree-A8 & 2.80 & 5.35 & 7.75 & 9.00 & 11.11 & 13.34 & 19.59 & 47.60 & 10.49 \\ \cmidrule(r){1-2} \cmidrule(lr){4-4} \cmidrule(lr){6-6} \cmidrule(lr){8-8} \cmidrule(l){10-10} 
% Quadtree-B8 & 4.14 &      & 8.21 &      & 12.26 &       & 28.94 &       & 17.51
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\centering
\begin{tabular}{l|ccccr}
Avg GT      & \multicolumn{1}{l}{50}       & \multicolumn{1}{l}{100}      & \multicolumn{1}{l}{150}      & \multicolumn{1}{l}{200}      & \multicolumn{1}{l}{All}  \\
Pair number & \multicolumn{1}{l}{731}      & \multicolumn{1}{l}{770}      & \multicolumn{1}{l}{722}      & \multicolumn{1}{l}{563}      & \multicolumn{1}{l}{2786} \\ \hline
RAFT (\cite{teed2020raft})      & 2.83 & 5.21 & 6.94 & 7.19 & 5.43                     \\ \hline
Linear (\cite{katharopoulos2020transformers})      & 2.87 & 5.05 & 6.96 & 7.96 & 5.56                     \\ \hline
SR (\cite{wang2021pyramid})  & \textbf{2.79} & 5.10 & 6.9  & 7.51 & 5.43                     \\ \hline
Quadtree-A (ours) & 2.94 & 5.09 & 6.96 & 7.15 & 5.42                     \\ \hline
Quadtree-B (ours) & 2.84 & \textbf{5.07} & \textbf{6.55} & \textbf{7.06} & \textbf{5.27}  
\end{tabular}
\caption{Results of optical flow estimation. We report end point error on frames sampled on ScanNet dataset. Compared with common used dataset like sintel and Kitti, this dataset contains more large displacement flow.}\label{tab:flow}
\end{table}

==> iclr2022/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> iclr2022/method_old.tex <==
\section{Method}
We first briefly review the attention mechanism in transformers in Section~\ref{sec:attn} and then  formulate our quadtree attention in Section~\ref{sec:quadtree_att}.


\subsection{Attention in Transformer}\label{sec:attn}
Vision transformers have shown great success in many tasks.
At the heart of a transformer is the attention module, which can capture long-range information between feature embeddings. 
Given two image embeddings $\mathbf{X}_1$ and $\mathbf{X}_2$, the attention module passes information between them. Self-attention is the case when $\mathbf{X}_1$ and $\mathbf{X}_2$ are the same, while cross attention covers a more general situation when $\mathbf{X}_1$ and $\mathbf{X}_2$ are different.
It first generates the query $\mathbf{Q}$, key $\mathbf{K}$, and value $\mathbf{V}$ by the following equation,
\begin{align*} 
\mathbf{Q}&=\mathbf{W}_q\mathbf{X}_1, \\ 
\mathbf{K}&=\mathbf{W}_k\mathbf{X}_2,\\
\mathbf{V}&=\mathbf{W}_v\mathbf{X}_2,
\end{align*}
where $\mathbf{W}_q$, $\mathbf{W}_k$ and $\mathbf{W}_v$ are learnable parameters. Then, it performs message aggregation 
% \ping{is `value aggregation' the correct name? We mentioned `message aggregation' at a few places.}
by computing the attention scores between query and key as following,
\begin{equation}
    \mathbf{Y}=\text{softmax}(\frac{\mathbf{Q}\mathbf{K^T}}{\sqrt{C}}) \mathbf{V^T},
    \label{equ:standard_transformer}
\end{equation}
where $C$ is the embedding channel dimension.
% The final step is to perform value aggregation.
% \begin{equation}
%     \mathbf{Y}=\mathbf{S}\mathbf{V^T}
% \end{equation}\label{equ:value}
The above process has $O(N^2)$ computational complexity, where $N$ is the number of image patches in a vision transformer. This quadratic complexity hinders transformers from being applied to tasks  requiring high resolution output. To address this problem, PVT (\cite{wang2021pyramid}) downsamples $\mathbf{K}$ and $\mathbf{V}$, while Swin-Transformer (\cite{liu2021swin}) limits the attention computation within local windows. 


\begin{figure}
\centering
    \includegraphics[width=0.95\textwidth]{iclr2022/image/quadtree_message.pdf}
  \caption{Illustration of quadtree message aggregation for a query token $q_i$. (a) shows the token pyramids and involved key/value tokens in each level. Attention scores are marked in the first two levels for clarification, and the top $K$ scores are highlighted in red. (b) shows message aggregation for QuadTree-A architecture. The message is assembled from different levels along a quadtree. (c) shows message aggregation for QuadTree-B architecture. The message is collected from overlapping regions from different levels.}
    \label{fig:quadtree_message}
\end{figure}

\subsection{QuadTree Attention}\label{sec:quadtree_att}
% Many computer vision tasks, e.g. image matching, optical flow estimation, stereo matching, require point-to-point costs. The computation of costs is similar to that of cross attention score. Empirical experiments show that leveraging self $+$ cross attention can significantly improve the performance.~\cite{} However, due to the large amount of points, existing works either use linear attention~\cite{} or attention with pooling to reduce the computation cost. This compromise can result in performance loss, since the point-to-point scores are not computed explicitly. 
In order to reduce the computational cost of vision transformers, we present QuadTree Attention. As the name implies, we borrow the idea from quadtrees, which are often used to partition a two-dimensional space by recursively subdividing it into four quadrants or regions. Quadtree attention computes attention in a coarse to fine manner. According to the results at the coarse level, irrelevant image regions are skipped quickly at the fine level. This design achieves less information loss while keeping high efficiency.

The same as the regular transformers, we first linearly project $\mathbf{X}_1$ and $\mathbf{X}_2$ to the query, key, and value tokens. To facilitate fast attention computation, we construct $L$-level pyramids for query $\mathbf{Q}$, key $\mathbf{K}$, and value $\mathbf{V}$ tokens respectively by $2\times 2$ average pooling. As shown in Figure~\ref{fig:quadtree}, after computing attention scores in the coarse level, for each query token, we select the top $K$ key tokens with the highest attention scores. At the fine level, query sub-tokens only need to be evaluated with those key sub-tokens that correspond to one of the selected $K$ key tokens at the coarse level. 
This process is repeated until the finest level. After computing the attention scores, we aggregate messages at all levels, where we design two architectures named as \textbf{QuadTree-A} and \textbf{QuadTree-B}.



% so that they should be divided for finer process like Quadtrees. 

% In contrast, quadtree attention adopt a coarse-to-fine strategy: 
%  \ping{This discussion is redundant. It can be removed to the introduction. The method section should focus on describing the method.}

% As the name implies, we borrow the idea from the quadtree, which is a tree structure with exactly four children. Quadtrees are often used to partition a two-dimensional space by recursively subdividing it into four quadrants or regions.
% For the query, key and value, we simply average pooling the projected embedding with a stride of two. 
% Each region (cell) in $l^{th}$ level covers four subregions (sub-cells) in $(l-1)^{th}$ level.

% The core idea is that for each query token at level $l$, we select $K^l$ tokens with the largest attention scores for finer computation. Therefore, for the next level, each query token  has $4\times K$ shared subregions to be processed. 
% The attention outputs are obtained between the query tokens and key tokens of the corresponding regions. 


% \begin{figure}
%     \includegraphics[width=0.3\textwidth]{iclr2022/image/quadtreeA_attn_score.pdf}
%   \caption{Illustration of attention score map for quadtree attention-A.}
%     \label{fig:quadtreeA_attn_score}
% \end{figure}


\textbf{QuadTree-A}. 
Considering the $i$-th query token $\mathbf{q}_i$ at the finest level, we need to compute its received message $\mathbf{m}_i$ from all key tokens. This design assembles the full message by collecting partial messages from different pyramid levels. Specifically, 
\begin{equation}
    \mathbf{m}_i = \sum_{1\leq l \leq L} \mathbf{m}_i^l,
\end{equation}
where $\mathbf{m}_i^l$ indicates the partial message evaluated at level $l$. This partial message $\mathbf{m}_i^l$ assemble messages
%skip top K related tokens while uses tokens 
at the $l$-th level from tokens within the region $\Omega_i^l$, which will be defined later. In this way, messages from less related regions are computed from coarse levels, while messages from highly related regions are computed in fine levels. This scheme is illustrated in Figure~\ref{fig:quadtree_message} (b),
% \ping{As shown in Figure~\ref{fig:quadtree_message} (b)}, 
message $\mathbf{m}_i$ is generated by assembling three partial messages that are computed from different image regions with different colors, which collectively cover the entire image space. The green region indicates the most relevant region and is evaluated at the finest level, while the red region is the most irrelevant region and is evaluated at the coarsest level. The region $\Omega_i^l$ can be defined as $\Gamma_i^{l} - \Gamma_i^{l+1}$, where the image region $\Gamma_i^l$ corresponds to the top $K$ tokens at the level $l-1$.  The regions $\Gamma_i^l$ are illustrated in  Figure~\ref{fig:quadtree_message} (c). The region $\Gamma_i^1$ covers the entire image.

The partial messages are computed as,
\begin{equation}
    \mathbf{m}_i^l = \sum _{j \in \Omega_i^l} s_{ij}^l \mathbf{v}_j^{l},
    \label{equ:att_score}
\end{equation}
where $s_{ij}^l$ is the attention score between the query and key tokens at level $l$. {Figure~\ref{fig:quadtree_message} (a) highlights query and key tokens involved in computing $\mathbf{m}_i^l$ with the same color as $\Omega_i^l$.}
Attention scores are computed recursively,
\begin{equation}
    s_{ij}^l = s_{ij}^{l-1} t_{ij}^l.
\end{equation}
Here, $s_{ij}^{l-1}$ is the score of corresponding parent query and key tokens and $s_{ij}^1 = 1$. The tentative attention score $t_{ij}^l$ is evaluated according to  Equation~\ref{equ:standard_transformer} among the $2\times 2$ tokens of the same parent query token.

%At the $l$-th level ($l>1$), the tentative attention scores are computed as,
%\begin{equation}
%    \mathbf{T}_{ij}^l=\text{softmax}(\frac{\mathbf{q}_i^l (\mathbf{K}^l_{\Lambda_{ij}^{l-1}})^\top} {\sqrt{C}}),
%    \label{equ:transformer_score}
%\end{equation}
%where $\Lambda_{ij}^{l-1}$ is the $j^{th}$ region in $\Lambda_{i}^{l-1}$ and $\mathbf{K}^l_{\Lambda_{ij}^{l-1}}$ is a matrix formed by stacking $2\times 2$ key tokens at level $l$ within the region  $\Lambda_{ij}^{l-1}$. 
%Then, we compute the final attention scores $S^{l}_{ij}$ in region $\Lambda_{ij}^{l-1}$ as
% \begin{equation}
%     s^{l}_{ij} = s^{l-1}_{ij} t_{ij}^{l}, \quad j \in \Lambda_i^{l-1}.
% \end{equation}
%\begin{equation}
%    \mathbf{S}^{l}_{ij} = s^{l-1}_{ij} \mathbf{T}_{ij}^{l},
%\end{equation}
%where $s^{l-1}_{ij}$ is the parent's attention score at level $l-1$. Effectively, this method redistribute the attention scores at coarse levels to fine levels. 
%redistribute the score of each block to finer level sub-blocks according to similarity $\text{sim}_{ij}^{l+1}$ of fine level query $\textbf{q}_i^{l+1}$and keys $\textbf{k}_j^{l+1}$, 
%where $\text{sim}_{ij}^{l+1}$ is computed as Equation~\ref{equ:transformer_score}. 


\textbf{QuadTree-B}. 
The attention scores $s_{ij}^l$ in \textbf{QuadTree-A} are recursively computed from all levels, which makes scores smaller at finer levels and reduces the contributions of fine image features. Besides,  fine level scores are also largely affected by the inaccuracy at coarse levels.
So we design a different scheme, referred as \textbf{QuadTree-B} in this paper, to address this problem. Specifically, we compute $\mathbf{m}_i$ as a weighted average of the partial messages from different levels, 
\begin{equation}
    \mathbf{m}_i = \sum_{1 \leq l \leq L} w_i^l \mathbf{m}_i^l,
\end{equation}
where $w_i^l$ is a learned weight. As shown in Figure~\ref{fig:quadtree_message} (c), the partial messages here overlap with each other, which are computed as,
\begin{equation}
    \mathbf{m}_i^l=\text{Attention}(\mathbf{q}_i^l, \mathbf{K}^l_{\Gamma _i^{l}}, \mathbf{V}^l_{\Gamma_i^{l}}),
    \label{equ:qudatreeB}
\end{equation}
where $\text{Attention}$ is the attention message computation as Equation~\ref{equ:standard_transformer}. Here, $\mathbf{K}^l_{\Gamma _i^{l}}$ and $\mathbf{V}^l_{\Gamma _i^{l}}$ are matrices formed by stacking all keys and values within the region $\Gamma_i^{l}$.

%For the coarse level, $\Gamma _l$ is the whole image, for finer levels, $\Gamma _l$ is the selected top-K region in each level as shown in Fig. \ref{}. 

%\jiahui{more explanation about B's advantage}

% Specifically, at level $l$, we do score computation and value aggregation with Eqn. \ref{equ:score} and Eqn. \ref{equ:value} among query tokens, the selected $4K$ key and value tokens. The final outputs are obtained by,
% \begin{equation}
% \mathbf{Y}=\sum_l w_l\mathbf{Y_l}
% \end{equation}
% \begin{equation}
%     \mathbf{W}=Softmax(\mathbf{P})
% \end{equation}
% where $\mathbf{Y_l}$ is the outputs of level $l$ and $w_i$ is $i^{th}$ element in $\mathbf{W}$. $\mathbf{P}$ is a set of learnable parameters, and we use softmax function to normalize them to get $\mathbf{W}$.

Both \textbf{QuadTree-A} and \textbf{QuadTree-B} involve only sparse attention evaluation. Thus, our method largely reduces computational complexity. As analyzed in Appendix~\ref{apx:complexity}, the computational complexity of our quadtree attention is linear to the number of tokens.

% \subsection{Complexity analysis}
% In this section, we analyze the computation complexity analysis of quadtree attention. Supposing the lengths of the query tokens, key tokens and value tokens are $H\times W$ and we have $L$ levels' token pyramids, the $l^{th}$ level has a token size of $\frac{H W}{4^(l-1)}$. The flops of computing quadtree attention is
% \begin{align*}
%      Flops&=2(\frac{H^2 W^2}{4^{L-1}}+\sum_{l-2}^{L-1}\frac{4KHW}{4^{l-1}}) \\
%      &=2(\frac{H^2 W^2}{4^{L-1}}+\frac{4}{3}(1-4^{1-L})KHW)
% \end{align*}.
% When $L$ approach infinite, the first $\frac{H^2 W^2}{4^{L-1}}+\sum_{l-2}^{L-1}$ approach 0, so $O(Flops)$ is equal to $O(KHW)$. Since $K$ is a constant number, the complexity of quadtree attention is linear to the number of tokens.
   


==> iclr2022/rebuttal.tex <==
We thank the reviewers for the valuable comments. We first present the guideline about our paper update, and then answer the questions of each reviewer.

1. Following PVTv2, we did not use positional encoding operation in the attention computation block for self attention tasks, while other works like Swin and Focal transformer already have positional encoding module.
After the paper submission, we augment our network with a multiscale positional encoding module (MPE), which is adapted from the locally-enhanced positional encoding [1]. The details are illustrated in Section 3.2, 'Multiscale position encoding'.
For objection detection, the AP can be improved by $1.3 - 1.6$ with our MPE module.
% negligible addition of flops and parameters. 
Results and more ablation studies are updated in the paper. 

[1] Cswin transformer: A general vision transformer backbone with cross-shaped windows. arXiv 2021.

2. More fair comparisons with other transformers. Due to limited time and resources, we give a comparison with PVTv2, Swin, Focal attention using a small model. More specifically, we replace the attention modules of PVTv2-b0 with these attention modules. Results are shown in Table. 5 of the latest paper. 
% More comparison will be added.



R1:
We thank for the very detailed and constructive suggestions.

\textcolor{red}{Q1: From the technical contribution aspect, the quadtree structure is not brand new. It is arguably true that the proposed approach is one of the earliest attempts to introduce quadtree structure into the attention mechanism. However, since some recent work [1] also employs coarse-to-fine structure in attention, it would be better to have some comparison with such work. [1] Focal Self-attention for Local-Global Interactions in Vision Transformers, NeurIPS 2021}

Answer: 
1. Comparison with Focal attention:
Focal attention is a concurrent work that also aims to capture both global and local attention in one single module, but is quite different from our work:
a) Focal attention only down-samples the key and value tokens and does not down-sample the query tokens when building multiscale attention, similar to the Poolingformer[1]. In contrast, we down-sample all these tokens. This can bring more efficiency in memory and computation since coarse level messages can be shared for the query sub-patches in the same patch, as shown in Fig. 1.


[1] Poolingformer: Long Document Modeling with Pooling Attention. ICML 2021.

b) Attention score and message generation. Focal attention concatenates all tokens from different levels in a single Softmax operator to compute the attention score and message. While our method computes the attention score and message separately at different levels. Thus, query tokens can share the same coarse level messages to reduce overhead.


c) Focal attention actually uses two-level attention in the released code. 
For high-resolution tasks like object detection, it covers about $1/6 \approx (15*7*4)^2 / (800*1333) $ size of the image in the first stage, even if windows size has been increased adaptively for COCO. While our method always covers the whole image.
Increasing the windows size or window level will result in larger memory consumption, although it already requires 2x memory than ours as shown in Tab. 5.
% for Focal attention because of the above memory and computation issue. 

%and it only covers an area of $49*49$ at most in one single operation, while our attention operation always covers the whole images. 
% From this point,  Focal attention is still a 'local' attention.
% A small attention window is not enough when using high-resolution images. So Focal transformer increase the window size to 
% As shown in the Tab.6 of the latest paper, our method is 2.4 higher than focal transformer in object detection on COCO (resolution $800 \time 1333$$), while only 0.3 higher in image classification in ImageNet (resolution $224 \time 224$)

d) Our work aims to design a general vision transformer not only for self attention tasks but also cross attention tasks. For cross attention tasks, the most related pixels in another image can be far away from the pixel itself, e.g., in the wide-baseline feature matching tasks shown in our paper. Thus, restricting the attention computation in a nearby window like Swin and Focal attention in a single attention computation might not be optimal for these tasks. Instead, we use the top K selection mechanism which allows the query tokens to attend dynamic regions in fine levels.

e) We give a comparison with Focal attention in classification and detection under the PVTv2-b0 setting. We achieve higher results especially in detection, where high-resolution images are required, with an improvement of 1.0 AP.

f) Focal attention is an arxiv paper when we submitted our paper into ICLR, and we did not notice it. We add discussions about it in the latest paper in Section 2, 'Vision Transformer'.



\textcolor{red}{Q2: The design of pyramid tokens is unclear:
(1) In Figure 1, Top-2 patches are used to compute finer attention. I wonder why in level 2 there are two sub-patches (green and yellow)? From the position of red patch in level, we should only have the green patch in level 2 (which could be consistent with Figure 2). In addition, why the two green patches in level 2 of image B have the same location in the 2x2 grid (both are lower left)? The same pattern is also observed in red patches in level 3.
(2) It remains unclear that how the pyramid tokens are generated: In Page 4-5, it mentions "we construct L-level pyramids for query and value V tokens respectively by 2x2 average pooling". Does it mean the coarse tokens are always average pooled fine tokens at one level lower? Is there any additional patch embedding layer introduced?
(3) In level 1, the top K patches are selected, which leads to 4K sub-patches in level 2. Does it uniformly sample top K sub-patches from 4K sub-patches, or each 2x2 sub-patches from coarse patch must have one sampled sub-patch?}

2. The design of token pyramid.
(1) 
a) \textit{there are two sub-patches (green and yellow) in the level2.} We show two sub-patches in level 2 to indicate that these two sub-patches share the same message computation in level 1. They have the same kNN patches, attention score and message. For level 3, we did not show more sub-sub-patches because of the complexity.

b) \textit{the two green patches in level 2 of image B have the same location.} This is a coincidence, they can be at random positions. We update Figure 1 to get rid of confusion.

c) *Does it uniformly sample top K sub-patches from 4K sub-patches*. No, we sample top K sub-patches according to the attention score, no other restricts are applied.

(2) Pyramid tokens generation. 
For QuadTree-A, we use average pooling for query, key and value tokens. For QuadTree-B, we use average pooling for query and key tokens, but for the value pyramid, we use convolution with stride 2 and normalization activation. This is also used in PVT and Focal transformer to down-sample key and value tokens. The total number of parameters is still less than other baselines, such as PVTv2. This value branch is useful for self attention tasks, but not for cross attention tasks. So only average pooling is used for cross attention tasks.
% (how about pvtv2 in feature matching????)
We make these issues clear in the latest submission.




\textcolor{red}{Q3:In the empirical experiments, the quadtree attention does not bring much efficiency improvement on the ImageNet classification: It has very similar #parameters and #flops compared with its baseline (PVTv2), which is quite different from the object detection task. I wonder what is the reason behind such as big gap.}

3. Efficiency improvement on object detection. The image resolution in COCO detection is much higher than ImageNet classification, $800 \times 1333$ vs $224 \times 224$. PVTv2 down-samples tokens by a fixed stride, which means the query token needs to compute attention with more key tokens when resolution is higher. While our method always computes attention with fixed top K tokens. Therefore, our method is more efficient when using higher resolution images.

4. Typos.

a) \textit{Equation (1): Should be V instead of V^T}: Yes.

b) \textit{Figure 2: It would be better to use \mathbf{m}_i^1 instead of m_i^1 for a consistent notation in the text.}: Yes.

c) \textit{Line below Eq (4): Should s_ij^1 be s_ij^0?}: No, we start from 1 as shown in Eq. 2. 

We fix these things in the latest submission. 


% % more similar to pooling former, P2T, belongs to local attention, no global attention, b) no query token pooling, coarse level message are shared in the same patch in our design, which is more efficient, more flops, c) can not be applied to cross attention, d) message generation is different. e) arxiv paper, recently noted)

% 2. figure1：level 2 green and yellow share the same knn patches.  patches has the same localization: it is a coincidence, ( a)figure 1 caption stress, b) coincidence, 

% 3. For B, newest version is that for q and k token parymid: only avg pooling, for value branch, convolution with stride 2 and normalization activation to add representation capability. Campared with PVT, our params is not increased. For quadtree-A, only avg pool. 

% 4. sample top K sub-patches from 4K sub-patches according to score instead of requiring 1 token every 2*2 patches. 

% 5. efficiency compaision with pvtv2.  object detection use large images, our method benifit more from large images

% typo:
% eq1.  yes
% fig2 yes

% eq4 bellow, no? we start from 1 as shown in eq2?





R2:
We thank for the valuable comments.

\textcolor{red}{Some important related works are missing. The previous work [1] also proposed a multi-level attention approach to efficiently balance the short-distance and long-distance attention, which proposed the same way to generate the multi-level or fine and coarse tokens. From this point, the idea of quadtreeB attention is very similar to [1]. However, the authors did not mention and discuss the relation to this very related work. I suggest the authors carefully discuss the relation [1].}

1. Comparison with Focal attention:
As the reply to R1.

\textcolor{red}{The paper proposed an efficient way to process long-distance and short-distance attention. There should be some baselines we should compare with, 1) the vanilla attention mechanisms, 2) some other efficient attention mechanisms, e.g. shifted windows attention in Swin-transformer, focal attention in Focal Transformer[1], sampled K, V in PVT. However, the authors only compared with the PVT. I'd like to see more solid apple-to-apple comparisons and discussions on that.}

2. Comparison with other transformers.
1) The vanilla attention mechanisms. We present a comparison with standard transformers in the stereo matching tasks. It achieves similar performance but is much more efficient. Due to limited resources, we did not give a comparison with the vanilla transformer on self attention task, e.g. ViT, since we have already compared with other recent efficient transformers. Besides, ViT is not suitable for high-resolution tasks like object detection.

2) Comparison with other efficient transformers.
a) Linear approximate attention. We give a comparison with Linear transformer on feature matching tasks as shown in Tab. 1. Our method is 2.7 higher in AUC@10$^{\circ}$.
b) Swin Transformer.
As shown in Tab. 5 of the latest submission, our method can achieve better results than Swin on both ImageNet and COCO, with an improvement of 1.4\% and 3.2\% AP respectively, which shows the effectiveness of global attention. 

c) Focal Transformer. As the previous reply.

% d) 'Sample K,V in PVT.': 
% Since our method has already been better than PVT, sampling K, V seems does not have advantage in improving the performance.

\textcolor{red}{Q1: How about the real runtime when applying quadtree attention to PVT architecture?}

3. Running time.

% Since we are not experts on CUDA programming. We implement quadtree attention with unoptimized CUDA codes, and thus current implementation is not efficient.
Currently, we only implement a naive CUDA codes without many optimizations, and it is not as efficient as the well-optimized dense GPU matrix operation.
We test the running time of Retinanet under PVTv2-b0 architecture. For PVTv2-b0, The running time is 0.026s to forward one image and for Quadtree-B-b0, the running time is 0.046s. However, Quadtree-B-b0 has much lower memory usage than PVTv2-b0. Quadtree-B-b0 consumes about 339 MB memory, while PVTv2-b0 consumes about 574 MB memory for one $800\times 1333$ image.
Further speed-up can be achieved by more engineering optimizations, such as {https://openreview.net/forum?id=agBJ7SYcUVb}.

\textcolor{red}{Q2: As I posted above, I think the quadtree attention mechanism is a general attention mechanism. I'd like to know how about the performance when applying to other transformer-based architecture, e.g. Swin-transformer, ViT, et. al.}

4. Comparison under other transformer  architecture.
As shown in Tab.8 in Appendix. E, we run Quadtree-B attention using Swin transformer architecture with the released codes. Our Quadtree-B attention obtains 82.2\% top 1 accuracy, 0.9\% higher than Swin transformer on ImageNet.

{Q3: The authors argue that Swin-transformer restricts the attention in the local windows. However, by shifting the windows in the Swin Transform, it enables that information exchange between windows for Swin. From this point, I don't think that Swin-transformer limits the attention within local windows.}

5. 
By saying \textit{Swin-transformer limits the attention within local windows}, we mean Swin computes attention in a local window in a single operation. Swin has to stack more blocks to capture long-range connections like CNN. We make it clear in the latest paper.




R3:
We appreciate for the constructive suggestions.

\textcolor{red}{Q1: Spare attention usually leads to a faster convergence rate, but higher final losses compared to full attention. I wonder if this still holds in QuadTree Attention. It is interesting to see the training curve of the proposed method compared with ViT or Swin.}

1. Convergence comparison with PVTv2 and Swin.
For the cross attention tasks, we provide training loss and testing accuracy curve in Fig.3 in the supplementary. QuadTree-B has larger training loss at first than PVT, then smaller loss in the final. But our method almost always has higher accuracy. 

For the self attention tasks, we provide training and validation accuracy curve of PVTv2-B0, Swin and our method in Figure 4. Our method achieves lower training loss and better validation accuracy all the time. 

\textcolor{red}{Q2: I wonder if the number of tokens in the finest resolution will affect the model performance. E.g., what is the current patch size of the input image, and will it lead to performance improvement if a larger or smaller patch size is chosen?}

2. \textit{patch size}.
We down-sample the image to 1/4 by a $7\times7$ convolution with a stride of 4, which means $4 \time 4$ sized patches are used. This is quite a common setting, ResNet/Swin/PVT all use this setting. 
% Current we do not provide results about changing the patch size. Experiments are ongoing if 

% After that we do not have 'patches' like ViT or Swin. Our QuadTree attention is applied on the entire image rather than patches.
\textcolor{red}{Q3: It is also worthy to explore if variants of larger (smaller) size in model parameters will lead to performance improvement, and how FLOPs change in these variants.}

3. 
\textit{model size.}
As shown in Tab. 3 and Tab. 4, we provide b0, b1, b2 networks with different model sizes, with a parameter number of 3.4M, 13.6M and 24.2M, a flop count of 0.6G, 2.2G, and 4.3G on ImageNet, and the top 1 accuracy is 71.9, 79.7 and 82.6. Due to limited resource, we will release results for larger models in the future.




R4:
\textcolor{red}{Q1: Top-k assignment for tokens in the quadtree is nondifferentiable, which may reduce the generalization. How does the proposed method achieve end-to-end training?}

1. Although top K is not differentiable, the gradient can also be passed to the selected query, key, value tokens, which enables end-to-end training. Top K selection is a common practice in network design, such as [1,2].

[1]: Kvt: k-nn attention for boosting vision transformers, arxiv 2021
[2]: Learning Camera Localization via Dense Scene Matching, CVPR 2021

\textcolor{red}{Q2: The quadtree aggregates features in an unstructured and iterative way. It is unfriendly to the parallel devices and probably takes more latency than the dense attention. It would be nice to provide the actual throughput on GPUs to demonstrate the efficiency.}
2. 
Currently, we only implement naive CUDA codes without many optimizations, and it is not as efficient as the well-optimized dense GPU matrix operation.
We test the running time of Retinanet under PVTv2-b0 architecture. For PVTv2-b0, The running time is 0.026s to forward one image and for Quadtree-b0, the running time is 0.046s for forwarding once. However, Quadtree-b0 has much lower memory usage than PVTv2-b0. Quadtree-b0 consumes about 339 MB memory, while PVTv2-b0 consumes about 574 MB memory for one $800\times 1333$ image.
Further speed-up can be achieved by more engineering optimizations, such as {https://openreview.net/forum?id=agBJ7SYcUVb}.


Paper update:
1. We update object detection results in Swin transformer setting in Table 8. 
In object detection, Quadtree attention is 2.6 higher than Swin. When compared with Focal Transformer, Quadtree attention obtains the same top 1 accuracy in image classification with fewer flops and 0.9 higher AP in object detection. 

2. We update comparison results with other transformers in the PVTv2-b0 setting.
For fair comparisons, we adopt the same positional encoding method LePE~\citep{dong2021cswin} for PVTv2, Swin and Focal transformer in Table 5. It is shown that quadtree attention obtain the best performance no matter what position encoding method is adopted.


For R1 and R2,
1. We have updated comparison results with other transformers in the PVTv2-b0 setting (Table 5) and Swin transformer setting (Table 8). For more fair comparison, we equip all transformers with the same position encoding methods (Table 5). In both settings, we achieve higher results than PVTv2, Swin and Focal Transformer.

2. Although we have already given comparison with Focal Transformer thoroughly in Table 5 and Table 8, 
it should also be noted that, according to the policy of ICLR review, it is not necessary to compare work available in Arxiv or publish within 4 months. 
% that Focal transformer is a concurrent work published in NeurIPS 2021. According to the policy of ICLR review, it is not necessary to compare work available in Arxiv or publish within 4 months. 




We conduct experiment using smaller patch size. Specifically, we down-sample the image to 1/8 by a  convolution with a stride of 8 and run the same PVTv2-b0. We observe a performance drop from 71.9 to 67.2. 


Sorry, we made a mistake in the main paper. $s_ij^1$ should be $S_ij^0$ and $S_ij^0=1$, level 0 is not exists and we represent the score of this level as $S_ij^0=1$ for the completeness of equation 4

==> iclr2022/related_work_old.tex <==
\section{Related work}

\textbf{Efficient Transformers.} Transformers have shown great success in both natural language processing and computer vision. Due to the quadratic computational complexity, the computation of full attention is unaffordable when dealing with long sequence tokens. Therefore, many works design efficient transformers, aiming to reduce computational complexity~\citep{katharopoulos2020transformers, choromanski2020rethinking, wang2020linformer, lee2019set, ying2018hierarchical}. Current efficient transformers can be categorized into three classes. 1) Linear approximate attention~\citep{katharopoulos2020transformers, choromanski2020rethinking, wang2020linformer, beltagy2020longformer, zaheer2020big} approximates the full attention matrix by linearizing the softmax attention and thus can accelerate the computation by first computing the product of keys and values.
%making use of the associativity property of matrix.
% Linear attention~\citep{katharopoulos2020transformers} treats the self-attention as a linear dot-product of kernel feature maps and make use of the associativity property of matrix products to reduce the complexity from $O(n^2)$ to $O(n)$. 
% Linformer~\citep{wang2020linformer}  demonstrate that the self-attention mechanism can be approximated by a low-rank matrix, and design a linear self-attention mechanism by decomposing the original scaled dot-product attention into multiple smaller attentions to approximate the low-rank matrix. 
% In contrast, performer~\citep{choromanski2020rethinking} estimate full-rank-attention by a novel fast attention via positive orthogonal random features approach. 
2) Inducing point-based linear transformers ~\citep{lee2019set, ying2018hierarchical} use learned inducing points with fixed size to compute attention with input tokens, thus can reduce the computation to linear complexity.
However, these linear transformers are shown to have inferior results than standard transformers in different works ~\citep{germain2021visual,chen2021learning}.
% , 2) sparse attention.~\cite{child2019generating, beltagy2020longformer, zaheer2020big, kitaev2020reformer}. 
3) Sparse attention, including Longformer~\citep{beltagy2020longformer}, Big Bird~\citep{zaheer2020big}, etc, attends each query token to part of key and value tokens instead of the entire sequence. Unlike these works, our quadtree attention can quickly skip the irrelevant tokens according to the attention scores at coarse levels. Thus, it achieves less information loss while keeps high efficiency.
% For example, Longformer~\citep{beltagy2020longformer} adopts a local windowed attention with a task motivated global attention. Big Bird~\citep{zaheer2020big} leverages graph sparsification methods that combines random attention, window attention and global attention together to reduce computation complexity. 
%Although those attentions are successful in NLP tasks, they are typically designed for self-attention instead of cross attention. 

\textbf{Vision Transformers.} Transformers have shown extraordinary performance in many vision tasks. ViT~\citep{dosovitskiy2020image} applies transformers to image recognition, demonstrating the superiority of transformers for image classification at a large scale. However, due to the computational complexity of full attention, it is hard to apply transformers in dense prediction tasks, e.g. object detection, semantic segmentation, etc. To address this problem, Swin-Transformer~\citep{liu2021swin} restricts attention computation in a local window.
Pyramid vision transformer (PVT)~\citep{wang2021pyramid} downsamples key and value tokens to reduce computation.
Although these methods have shown improvements in various tasks, they have drawbacks either in capturing long-range dependencies ~\citep{liu2021swin} or fine level attention ~\citep{wang2021pyramid}.
The K-NN transformers~\citep{wang2021kvt, zhao2019explicit}  aggregate messages from top $K$ most similar tokens as ours, but they compute the attention scores among all pairs of query and key tokens, and thus still has quadratic complexity. 

Beyond self-attention, many tasks can largely benefit from cross attention. Superglue~\citep{sarlin2020superglue} processes detected local descriptors with self- and cross attention and shows significant improvement in feature matching. Standard transformers can be applied in SuperGlue because only sparse keypoints are considered. SGMNet ~\citep{chen2021learning} further reduces the computation by attending to seeded matches. LoFTR~\citep{sun2021loftr} utilizes linear transformer~\citep{katharopoulos2020transformers} on low-resolution feature maps to generate dense matches.
For stereo matching, STTR ~\citep{li2020revisiting} applies self- and cross attention along epipolar lines and reduces the memory by gradient checkpointing engineering techniques.
However, due to the requirement of processing a large number of points, these works either use linear transformers, which compromise performance, or a standard transformer, which compromises efficiency. In contrast, our transformer with quadtree attention achieves a significant performance boost compared with linear transformer or efficiency improvement compared with standard transformer. Besides, it can be applied to both self-attention and cross attention.

\input{iclr2022/tree_structure}


==> iclr2022/segmentation_table.tex <==
\begin{table}[]
\centering
\small
\begin{tabular}{l|lll}
              & \#Param (M) & GFlops & mIoU \\ \hline
PVTv2-b0      & 7.6         & 25.0       & 38.6 \\
QuadTree-B-b0 & \textbf{7.5}         & \textbf{24.6}   & \textbf{39.9} \\ \hline
PVTv2-b1      & 17.8        & 34.2       & 42.3 \\
QuadTree-B-b1 & \textbf{17.4}        & \textbf{33.8}   & \textbf{44.7} \\ \hline
PVTv2-b2      & 29.1        & 45.8      & 47.9 \\
QuadTree-B-b2 & \textbf{28.8}        & \textbf{45.4}   & \textbf{48.7}\\ \hline
PVTv2-b3      & \textbf{49.0}        & \textbf{62.4}       & 49.0 \\
QuadTree-B-b3 & 50.0        & 63.1   & \textbf{50.0} \\ \hline
PVTv2-b4      & \textbf{66.3}        & \textbf{81.3}       & 49.3 \\
QuadTree-B-b4 & 68.0        & 82.6   & \textbf{50.6}
\end{tabular}
\caption{Semantic segmentation performance of different backbones on the ADE20K validation set. We use semantic-FPN as the general framework for semantic segmentation.}\label{tab:sematic_seg}
\end{table}

==> iclr2022/tree_structure.tex <==
\textbf{Tree structure.} Many works adopt quadtree or octree structure~\citep{riegler2017octnet, wang2017cnn, jayaraman2018quadtree, sullivan1994efficient, spann1985quad, samet1984quadtree} to accelerate data processing time by focusing on the interesting subsets of data. 
% Quadtree or octree are often used to partition a two-dimensional or three-dimensional space by recursively subdividing it into four or eight regions. 
% In computer vision, these structures are used to skip unimportant regions. 
For example, in 3D object recognition tasks, \cite{riegler2017octnet} hierarchically partitions the 3D space using a set of unbalanced octrees 
% where each leaf node stores a pooled feature representation. This design allows focusing 
to focus computation to the relevant dense regions. \cite{jayaraman2018quadtree} decomposes and represents the image as a linear quadtree that is only refined in the non-empty portions of the image. Following the spirit of these works, our quadtree attention quickly skips irrelevant regions in the fine level according to the results in the coarse level. \jiahui{can delete this section if no more space}
